A Krylov projection algorithm for large symmetric matrices with dense spectra

We consider the approximation of $B^T (A+sI)^{-1} B$ for large s.p.d. $A\in\mathbb{R}^{n\times n}$ with dense spectrum and $B\in\mathbb{R}^{n\times p}$, $p\ll n$. We target the computations of Multiple-Input Multiple-Output (MIMO) transfer functions for large-scale discretizations of problems with continuous spectral measures, such as linear time-invariant (LTI) PDEs on unbounded domains. Traditional Krylov methods, such as the Lanczos or CG algorithm, are known to be optimal for the computation of $(A+sI)^{-1}B$ with real positive $s$, resulting in an adaptation to the distinctively discrete and nonuniform spectra. However, the adaptation is damped for matrices with dense spectra. It was demonstrated in [Zimmerling, Druskin, Simoncini, Journal of Scientific Computing 103(1), 5 (2025)] that averaging Gau{\ss} and Gau\ss -Radau quadratures computed using the block-Lanczos method significantly reduces approximation errors for such problems. Here, we introduce an adaptive Kre\u{i}n-Nudelman extension to the (block) Lanczos recursions, allowing further acceleration at negligible $o(n)$ cost. Similar to the Gau\ss -Radau quadrature, a low-rank modification is applied to the (block) Lanczos matrix. However, unlike the Gau\ss -Radau quadrature, this modification depends on $\sqrt{s}$ and can be considered in the framework of the Hermite-Pad\'e approximants, which are known to be efficient for problems with branch-cuts, that can be good approximations to dense spectral intervals. Numerical results for large-scale discretizations of heat-diffusion and quasi-magnetostatic Maxwell's operators in unbounded domains confirm the efficiency of the proposed approach.

==> Numerics.tex <==

\section{Numerical Examples}\label{sec:NumEx}

{\color{red} In this section, we consider the application of the developed error bounds and {\clr show that} the {\clr averaging} formulas {\clr accelerate convergence} for MIMO transfer function computations for PDE operators with continuous or very dense spectrum when Krylov subspace approximations lose their spectral adaptivity. This phenomenon can only be observed for large-scale problems, thus dimensions of our experiments are of order $10^5-10^6$. Though the theory in this manuscript is limited to the resolvent with $s\in \mathbb{R}^+$, we stress that the error bound, monotonicity and {\clr error correction via averaging} seem to hold for imaginary $s$ and other functions such as $\phi(A)=\exp(-A t)$. We also explore possible accelerations stemming from adding random vectors to the initial block.
All errors reported are measured in the 2-norm. }




\subsection{Transfer functions of PDE operators on unbounded domains}\label{sec:PDE}
The proposed approach focuses on computing transfer functions for matrices with dense spectra, e.g.  self-adjoint PDE operators in unbounded domains, particularly for matrices with dense spectra. To achieve accurate PDE discretization in such settings, we employ the optimal grid approach (\cite{idkGrids}), which ensures spectral convergence in the exterior region of the computational domain. For a more detailed discussion on the implementation of optimal grids, see \cite{druskin2016near}. A key consequence of using spectral approximation for the exterior problem is that the spectrum of $A$. A closely approximates the continuous spectrum of the original problem, reducing the adaptability of Krylov subspace approximations.

\subsubsection{2D Diffusion}\label{sec:subsubsection2D}
We discretize the operator  
\[
\sigma({\bf x})^{-\frac{1}{2}}\Delta\sigma({\bf x})^{-\frac{1}{2}}
\]
on an unbounded domain using second-order finite differences over a $300\times 300$ grid. In the central region of the grid, where $\sigma(\bx)$ varies, we set the grid spacing to $\delta_x=1$.  

{ This formulation is relevant to both heat transfer and the scalar diffusion of electromagnetic fields. To approximate the problem numerically, we impose a Dirichlet boundary condition on a bounded domain, employing $N_{opt}=10$ exponentially increasing grid steps in the exterior while maintaining a uniform grid in the interior. By using the optimal geometric factor $\exp{(\pi/\sqrt{10})}$, as suggested in \cite{idkGrids}, we achieve spectral accuracy in the exterior region, effectively approximating the boundary condition at infinity through exponential decay.}  

The resulting grid and function $\sigma(\bx)$ are illustrated in Figure~\ref{fig:Heat2config}. The figure only depicts the first two steps of the exponentially increasing grid, as subsequent steps grow rapidly. Here, $B$ is represented as a vector of discrete delta functions with nonzero entries at the grid nodes corresponding to the transducer locations, labeled as {\it Trx} in the figure.  

Figure~\ref{fig:HeatReal} presents the convergence results for $s=10^{-3}$, while Figure~\ref{fig:HeatImag} shows the convergence behavior for purely imaginary shifts $s=\imath\cdot10^{-3}$. In the latter case, block Lanczos exhibits slower convergence. { The monotonicity result in Theorem~\ref{lem01} and the error bound in equation~(\ref{eq:ErrorBound}) are rigorously established only for $s\in\mathbb{R}^+$.} Nevertheless, in this example, the convergence for purely imaginary $s$ remains monotone, the upper bound holds, and {averaged quadrature rules} reduce the approximation error by an order of magnitude. For the selected shifts, both { averaging formulas} perform equally well.


\begin{figure}[h!]
	\centering
	% \includegraphics[width = \linewidth]{7_Diffusion_gridopt/Grid.pdf}
	\includegraphics[width = 0.65 \linewidth]{2_Grid.png}
	\caption{Grid, head conductivity $\sigma(\bx)$ and transducer locations of the heat diffusion textcase.}\label{fig:Heat2config}
\end{figure}



\begin{figure}[h!]
	\centering	
	\begin{subfigure}[b]{.48\linewidth}
		\centering
		%\includegraphics[width = \linewidth]{7_Diffusion_gridopt/Extrapolation_s_r0_i0.001.pdf}
		%\includegraphics[width = \linewidth]{02_Convergence_imag_s_0_001.pdf}
		\caption{Error norms  for {\bf imaginary} $s=0.001i$.}\label{fig:HeatImag}
	\end{subfigure}
	\begin{subfigure}[b]{.48\linewidth}
		\centering
		% \includegraphics[width = \linewidth]{7_Diffusion_gridopt/Extrapolation_s_r0.001_i0.pdf}
%		\includegraphics[width = \linewidth]{Z_02_AntiGauss_Convergence_s_r0.001_i0.pdf}
		\caption{Error norms for {\bf real} shift $s=0.001$}\label{fig:HeatReal}
	\end{subfigure}%
	
	\begin{subfigure}[b]{.48\linewidth}
		\centering
		%\includegraphics[width = \linewidth]{7_Diffusion_gridopt/EXP_Extrapolation_TimeDom_t_10000.pdf}
		%\includegraphics[width = \linewidth]{02_Convergence_Exp_t_10000.pdf}
		\caption{Error norms for the exponential function $\phi(A)=\exp{(-At)}$ for $t=10000$.}\label{fig:HeatExp}
	\end{subfigure}
	
	
	\caption{Convergence and {\clr quadrature rule averaging} for the 2D heat diffusion problem. }
\end{figure}

\subsubsection{3D Electromagnetic diffusion}\label{sec:EMdiff} In this example, we consider the solution of the 3D Maxwell equations in the quasi-stationary (diffusive) approximation. Krylov subspace methods for approximating the action of matrix functions in this context were first introduced in \cite{druskin1988spectral} and remain a widely used approach in geophysical applications. The diffusive Maxwell equations in $\mathbb{R}^{3}$ can be rewritten as  
\be\label{eq:max}
(\nabla \times \nabla \times +\sigma(\bx) \mu_0 s)\mathcal{E}_{(r)}(\bx,s) = - { s}\mathcal{J}^{\rm ext}_{(r)}(\bx,s), \quad \bx\in \Omega,
\ee  
where $\sigma$ represents the electrical conductivity, $\mu_0$ is the vacuum permeability, and $\mathcal{J}^{\rm ext}_{(r)}$ is the external current density associated with the transmitter index $(r)$, generating the electric field $\mathcal{E}_{(r)}(\bx,s)$. For $s\notin\mathbb{R}_-$, the solution of \eqref{eq:max} vanishes at infinity,  
\be\label{eq:inftymax}  
\lim_{\bx\to\infty} \|\mathcal{E}(\bx)\|=0.  
\ee  

To approximate \eqref{eq:max}-\eqref{eq:inftymax}, we employ the conservative Yee grid, following the methodology outlined in \cite{druskin1988spectral}. Similar to the approach used for the diffusion problem in $\mathbb{R}^2$, we truncate the computational domain by imposing Dirichlet boundary conditions on the tangential components of $\mathcal{E}_{(r)}$ at the boundary. The grid is constructed with an optimally spaced geometric progression, ensuring spectral convergence of {\clr condition~\eqref{eq:inftymax} at infinity}. In our setup, we use $N_{opt}=6$ geometrically increasing grid steps with a scaling factor of $\exp{(\pi/\sqrt{6})}$, as proposed in \cite{idkGrids}. The resulting grid consists of $N_x=80$, $N_y=100$, and $N_z=120$ points, yielding a matrix $A$ of size $N=2\,821\,100$.  

The conductivity $\sigma$ is homogeneous and set to $1$ throughout the domain, except for two inclusions where $\sigma=0.01$, as depicted in Figure~\ref{fig:4_config}. The excitation consists of six magnetic dipoles (approximated by electric loops): three positioned above the inclusions and three located at their center, as indicated by the arrows in Figure~\ref{fig:4_config}. This setup is analogous to tri-axial borehole tools used in electromagnetic hydrocarbon exploration \cite{saputra2024adaptive}, leading to a matrix $B$ with six columns.  

%The operator and its discretization are nonnegative definite; however, since the columns of $B$ correspond to divergence-free magnetic sources, they are inherently orthogonal to the null space of the operator, which consists of potential solutions. Consequently, the conditions outlined in Remark~\ref{rem:Nullspace} are satisfied.  

%Figure~\ref{fig:EMSweeps} illustrates the convergence for various real values of $s$ after $m=400$ block iterations, demonstrating that the error bound remains tight across all values of $s$ and that there is no difference in {\clr averaging} formulas. Furthermore, Figure~\ref{fig:EM_conv_Real} shows the convergence behavior for a real shift of $s=0.05$, while Figure~\ref{fig:EM_conv_Imag} presents the results for an imaginary shift.% of $s=0.1 \imath$.

%results:
%C:\Users\jorzi493\Box\Matlab\KreinNudelman\PaperVersion\MIMO_Results\Paper\7_Diffusion_gridopt_BS
% rerun full convergence?
%C:\Users\jorzi493\Box\Matlab\KreinNudelman\PaperVersion\Results\Paper


\begin{figure}[h!]
 \centering
 
 \begin{subfigure}[b]{.47\linewidth}
 \centering
 \includegraphics[width = 0.75\linewidth]{4_Config.png}
 \caption{3D rendering of the simulated configuration with two inclusions.}
 \label{fig:4_config}
 \end{subfigure}%
 \hspace{1em}
 \begin{subfigure}[b]{.47\linewidth}
 \centering
 % \includegraphics[width = \linewidth]{11_EM3D/sSweep_Iter400Freqs_r0.01_i0.pdf}
 %\includegraphics[width = \linewidth]{4_SweepS_it400.pdf}
 \caption{Error norms for various values of $s$ after $m=400$ iterations.}
 \label{fig:EMSweeps}
 \end{subfigure}
 
 \begin{subfigure}[b]{.47\linewidth}
 \centering
 %\includegraphics[width = \linewidth]{11_EM3D/Extrapolation_s_r0.05_i0.pdf}
 %\includegraphics[width = \linewidth]{4_Convergence_real_s_0_05}
 \caption{Error norms with real shift $s=0.05$. \phantom{force line break}}
 \label{fig:EM_conv_Real}
 \end{subfigure}%
 \hspace{1em}
 \begin{subfigure}[b]{.47\linewidth}
 \centering
 %\includegraphics[width = \linewidth]{11_EM3D/Extrapolation_s_r0_i0.1.pdf}
 %\includegraphics[width = \linewidth]{4_Convergence_imag_s_0_1}
 \caption{Error norms with {\rm imag.} shift $s=0.1\imath$.}
 \label{fig:EM_conv_Imag}
 \end{subfigure}%
\caption{Convergence of the block Lanczos method and {\clr XXX} 3D electromagnetic case.}
\end{figure}

\iffalse
 \subsection{Graph Laplacian}\label{sec:graphL} {\color{red} Efficient computation of SISO and MIMO transfer functions of large graph-Laplacians is important for efficient clustering of big data sets, computation of centrality measures and other applications \cite{lot2008,Benzi2020MatrixFI,druskin2022distance}. For our numerical experiments we} take the \texttt{web-BerkStan} graph from the SNAP (Standford network analysis project) \cite{snapnets} and turn it into an undirected graph by symmetrization. The original graph has 685230 nodes and 7600595 edges and we construct the normalized graph Laplacian $A$ as our test matrix. The nodes of the graph represent pages from berkeley/stanford.edu domains and directed edges (here converted to undirected edges) represent hyperlinks between them. The data were collected in 2002. 
 
As $B$ matrix we take $p=3$ (graph) delta functions chosen at random nodes\footnote{With random seed 1 we obtain delta functions at nodes 207168, 100562, and 63274.}. The graph Laplacian is nonnegative definite, where the null space of the graph Laplacian consists of constant vectors on every connected graph component.  The columns of $B$ are graph delta functions in our experiments and thus not orthogonal to the null space; however, excluding the case of connected graph components of dimension 1 (single disconnected nodes), the column space of $B$ intersects trivially with the null space of $A$, and as such, satisfies the condition of Remark~\ref{rem:Nullspace}.
 
 In Figure~\ref{fig:GraphLap} we evaluate the resolvent $\phi(A,s)=(A+s I)^{-1}$ for $s=10^{-4}$ showing that the error bound is tight and the {\clr averaging} formulas give similar results. After $m=50$ block iterations the error for various values of $s$ is displayed in Figure \ref{fig:GraphLap2}.
 
 
 
 \begin{figure}[h!b]
 	\centering
 	\begin{subfigure}[b]{.48\linewidth}
 		\centering
 		\includegraphics[width = \linewidth]{X3_Graph_Convergence_Deltas_s=0_0001.pdf}
 		\caption{Error norms with shift $s=10^{-4}$. \phantom{just force a line break}}
 		\label{fig:GraphLap}
 	\end{subfigure}~
 	\begin{subfigure}[b]{.48\linewidth}
 		\centering
 		\includegraphics[width = 0.93\linewidth]{X3_Graph_Delta_Iter50_s=0_01.pdf}
 		\caption{Error norms after $m=50$ iterations for various values of $s$.}
 		\label{fig:GraphLap2}
 	\end{subfigure}%
 	\caption{Convergence, error bound and {\clr averaged quadrature rules} for the normalized graph Laplacian test case}
 \end{figure}
 
 {\color{red} In contrast to PDE operators on unbounded domains, data-related graphs may exhibit spectral distributions with non-vanishing gaps even at very large dimensions. Consequently, they cannot be regarded as approximations of the problems discussed in Proposition~\ref{prop:corr}. Nevertheless, as illustrated in Figure~\ref{fig:GraphLap}, quadrature approximations for such graphs can demonstrate linear convergence, in which case they satisfy tight block Gauss-Radau bounds and their {\clr averaging} will be efficient. }
 \fi
